Delta State Replicated Data Types

CRDTs are distributed data types that make eventual consistency of a distributed object possible and non ad-hoc. Specifically, state-based CRDTs ensure convergence through disseminating the entire state, that may be large, and merging it to other replicas; whereas operation-based CRDTs disseminate operations (i.e., small states) assuming an exactly-once reliable dissemination layer. We introduce Delta State Conflict-Free Replicated Data Types ($\delta$-CRDTs) that can achieve the best of both worlds: small messages with an incremental nature, as in operation-based CRDTs, disseminated over unreliable communication channels, as in traditional state-based CRDTs. This is achieved by defining delta mutators to return a delta-state, typically with a much smaller size than the full state, that to be joined with both local and remote states. We introduce the $\delta$-CRDT framework, and we explain it through establishing a correspondence to current state-based CRDTs. In addition, we present an anti-entropy algorithm for eventual convergence, and another one that ensures causal consistency. Finally, we introduce several $\delta$-CRDT specifications of both well-known replicated datatypes and novel datatypes, including a generic map composition.

==> algo.tex <==
\subsection{Algorithms}
\label{subs:algo}
Section~\ref{sec:shipping} investigated that eventual convergence of \dsrdt can by maintained by any anti-entropy protocol (AEP) that can eventually deliver all the deltas of a replica to other replicas. We intentionally kept this requirement quite generic to allow for a greater number of AEP already present in communication systems. In this section, however, we introduce two basic algorithms that define the minimal requirements required by an AEP to maintain eventual consistency in \dsrdt. The two protocols show how to use use delta shipping with or without maintaining the causal order of operations depending on the semantics demanded. Both algorithms can be used as \textit{plug-ins} in an anti-entropy protocol. 

\begin{figure}
\centering
\colorbox{light-gray}{
\begin{minipage}[c]{.45\textwidth}
\centering
    \include{basic-algo}
    \label{subf:non-causal}
\end{minipage}
~
\begin{minipage}[c]{.45\textwidth}
\centering
    \include{causal-algo}
    \label{subf:causal}
\end{minipage}}
\caption{$\delta$-SRDT distributed algorithm for replica $i$, for the
crash-recovery asynchronous network model.}
\label{fig:algo}
\end{figure}

\subsubsection{Basic Non-Causal Algorithm}
A basic non-causal distributed algorithm to be used at the node corresponding to replica $i$ is
presented in Figure~\ref{fig:algo}. The durable state, which persists
after a crash, is simply the \dsrdt state $X_i$.
Volatile state $D$ from the same join-semillatice -- a delta-group -- is
used to accumulate deltas before eventually sending it to other replicas.
We assume for convenience and WLOG that the join-semilattice has a bottom,
which is the initial value for both $X_i$ and $D_i$. (It is always possible to
add a bottom to a bottomless join-semilattice and add a family of mutators to
move into what would be an arbitrary initial state otherwise.)




When an operation, given by some mutator $m^\delta$ is performed, the mutator
is applied to the current state, generating a delta $d$. This delta is joined
both with the current \dsrdt state, to produce the next state, and into $D$.

In the same spirit of standard state based CRDTs, a node does not send
messages to others after every data-type operation, but only from time to
time, what we denote in the algorithm by \emph{periodically}. When sending a
message, the payload is either the delta-group $D_i$ or the full state $X_i$.
The decision is left to another parameter of the algorithm: function $\af{choose}_i$,
 which returns one of them. This basic algorithm does not
attempt to distinguish neighbors, and just effectively broadcasts the same
message to all. In any case, after a send, the delta-group is reset to bottom.

When a message is received, the payload $d$ is joined into the current \dsrdt
state.  The basic algorithm can operate in one of two modes of operation: in
the \emph{transitive} mode (when $t_i$ is true) $m$ is also joined into $D$,
allowing transitive propagation of delta-mutations (deltas received at $i$
from some node $j$, can later be sent to some other node $k$); in the
\emph{direct} mode, a delta-group is the join of exclusively local
delta-mutations (in the same example, $j$ would have to send its deltas
directly to $k$).

The decisions of whether to send a delta-group versus (typically less
periodically) sending the full state, and whether to use transitive or direct
mode  can be made according to state size, message loss distribution
assumptions, and network topology. 
%Regardless of these parameterization possibilities, given this basic algorithm, we have the following simple result.

\subsubsection{Causal Algorithm}

We now present a distributed algorithm to be used with \dsrdt{}s, which
enforces the causal delta-merging condition, to be used whenever the causal
consistency guarantees of standard state-based CRDTs are needed.
Figure~\ref{fig:algo} is the canonical version, before important
optimizations which we leave to Section~\ref{TODO}. It distinguishes neighbor
nodes and sends them only delta-intervals that when joined at the receiving
node will obey the delta-merging condition.

Each node $i$ keeps a contiguous sequence of deltas $d_i^m, \ldots, d_i^M$ in
a map $D$ from integers to delta-states (with at any point, $m =\min(\dom(M))$ and $M = \max(\dom(M))$.  Delta sequence numbers are obtained
through a counter $c_i$ which is incremented after each delta (either
delta-mutation or delta-interval received).

Each node $i$ keeps also an acknowledge map $A$ that, for each neighbor $j$
stores the highest $b$ such that a delta interval $\dint iab$ that $i$ sent to
$j$ was definitely joined into $X_j$.
Each node $i$ sends some delta-interval $d=\dint iab$ with a $(\af{delta}, d,
b)$ message; the receiving node $j$, after joining $\dint iab$ into its replica
state, will reply with an acknowledgement message $(\af{ack}, b)$; when receiving
the ack from $j$, node $i$ will update the $j$ entry in the acknowlege
map, using the max funtion, to cope with possible old duplicates or in general
messages arriving out of order.

Like the \dsrdt state, the counter $c_i$ is also kept in durable storage; this
is so that after a crash and recovery there is no danger of different deltas
generated in two ``epochs'' using the same sequence number.
Otherwise, there would be the danger of some (possibly duplicate) ack for a
delta-interval that was sent before crashing could lead to a node violating
the delta-merging condition by skipping the sending of some deltas generated after
the recovery.

The algorithm for node $i$ periodically picks a random neighbor $j$ and, if
the sequence of deltas is empty or the oldest still kept delta is more recent than
what can be sent to $j$ according to acks received from $j$ (e.g., after a
crash and recovery) node $i$ will send the full state; otherwise, it will send
the join of all deltas, from the number that $j$ acked (an ack if for the
lower range of an interval that can be sent) up the the more recent.
The algorithm also periodically garbage collects the sequence of deltas,
removing all deltas that have been acked by all neighbors.


==> mathdefs.tex <==
\RequirePackage{latexsym}
\RequirePackage{dsfont}

% macros for domain teory, semantics, etc. 

% math code definitions

%%%%%%%%%%%%%%%%%%%%%%%%\mathcode`:="603A          % : as punctuation
\mathcode`.="613A          % . as punctuation
\mathcode`|="326A          % | as a relation

\let\es=\relax    %  possible space before punctuation in displayed formulas

%% relations

\newcommand\tx[1]{\hbox{ #1 }}
\newcommand{\defeq}{\stackrel{.}{=}}

\let\vect=\overrightarrow
\let\iff=\Leftrightarrow        % this redefines the original
\let\implies=\Rightarrow
\let\implied=\Leftarrow

\let\sqleq=\sqsubseteq
\let\sqgeq=\sqsupseteq
\let\pleq=\sqleq          % partial-order leq
\let\ple=\sqsubset          % partial-order le
\let\pgeq=\sqgeq          % partial-order geq

\def\land{\mathrel{\wedge}}
\def\lor{\mathrel{\vee}}
\let\bigland=\bigwedge
\let\biglor=\bigvee

\def\preleq{\mathrel{%      % pre-order leq
  \raise 2pt\hbox{$\mathop\sqsubset\limits_{\hbox{$\sim$}}$}%
}}

% operators

\let\union=\cup
\let\bigunion=\bigcup
\let\join=\sqcup
\let\bigjoin=\bigsqcup
\let\meet=\sqcap
%\let\bigmeet=\bigsqcap
\newcommand{\down}{\mathord{\downarrow}}

\newcommand\setsize[1]{\left| #1 \right|}
\newcommand\domxtn{\mathbin{\stackrel{+}{|}}}
%\newcommand\domsub{\mathbin{\stackrel{-}{|}}}
\newcommand\domainsub{\mathop{\lhd\mkern-14mu-}}

% arrows

\newcommand{\map}{\mathrel{\hookrightarrow}}
\newcommand\goesto[1]{{\mathop{\longrightarrow}\limits^{#1}}}
\newcommand\goes{\longrightarrow}

% function constants

\newcommand\auxfun[1]{\expandafter\newcommand\csname #1\endcsname{%
 \mathop{\hbox{$\mathsf{#1}$}}\nolimits}}
 \newcommand\af[1]{\mathop{\hbox{$\mathsf{#1}$}}\nolimits}
 \newcommand\kw[1]{\mathrel{\hbox{$\mathbf{#1}$}}}

\let\max=\relax
\auxfun{max}
\auxfun{Max}
\auxfun{fix}
\auxfun{dom}
\auxfun{fst}
\auxfun{snd}
\auxfun{ran}

% sets

\newcommand{\pow}[1]{{\cal P}(#1)}
\newcommand{\unit}{\mathds{1}}
\newcommand{\bool}{\mathds{B}}
\newcommand{\nat}{\mathds{N}}
\newcommand{\integer}{\mathds{Z}}
\newcommand{\ids}{\mathds{I}}

\newcommand{\false}{\mathsf{False}}
\newcommand{\true}{\mathsf{True}}

%%%%%%%%%%%

\newcommand\letin[2]{\mathop{\hbox{$\mathrm{let}$}} #1 \Leftarrow #2 . }
\newcommand\lift[1]{\lfloor #1 \rfloor}

%%%%%%%%%%%%%%%%%%%%%

\newcommand\iffdef{\mathrel{\Longleftrightarrow}}
\newcommand\nullstring{\epsilon}
\newcommand\pfunc{\hookrightarrow}
\newcommand\func{\rightarrow}


